Quantifying the Effect of Matrix Structure on Multithreaded Performance of the SpMV Kernel

Sparse matrix-vector multiplication (SpMV) is the core operation in many common network and graph analytics, but poor performance of the SpMV kernel handicaps these applications. This work quantifies the effect of matrix structure on SpMV performance, using Intel's VTune tool for the Sandy Bridge architecture. Two types of sparse matrices are considered: finite difference (FD) matrices, which are structured, and R-MAT matrices, which are unstructured. Analysis of cache behavior and prefetcher activity reveals that the SpMV kernel performs far worse with R-MAT matrices than with FD matrices, due to the difference in matrix structure. To address the problems caused by unstructured matrices, novel architecture improvements are proposed.

==> PFMR.tex <==
\subsection{Prefetcher Miss Rate}

\begin{figure}[htb]
        \centering       
        \includegraphics[width=0.49\textwidth]{images/PFMR.png} 
        \caption{Prefetcher Miss Rate of the SpMV kernel on FD matrices (blue) and R-MAT matrices (red) in serial and in parallel.}
        \label{fig:PFMR}
\end{figure}



Figure~\ref{fig:PFMR} 

Prefetcher activity --> L2 stall cycles

==> datasets.tex <==
\subsection{Datasets}

We analyze the SpMV kernel for two types of matrices: one somewhat
structured and one highly unstructured. Structured matrices allow the
SpMV kernel to make better use of the cache structure. Unstructured
matrices, however, result in the SpMV kernel making many cache misses
and generally not using cache to speed up computation. For a baseline
to compare peformance too, dense matrices are also included.

FD matrices are used to represent somewhat structured matrices. These
matrices are generated using two-dimensional finite difference
method. The resultant matrices consist of three diagonal bands of
three elements each, which means that FD matrices have nine elements
per row.

To respresent unstructured matrices, R-MAT matrices~\cite{rmat} are
used. R-MAT matrices are constructed to approximate realistic network
models using a powr law distribution. This distribution naturally
creates a skew in the distribution of nonzeros, leading to
difficulties in effective load balancing to allow easy comparison to
SpMV performance on FD matrices. To counteract this, the rows and
columns of the R-MAT matrices are randomly permuted. This does not
impact the problem represented by the matrix, but allows a uniform
block distribution to easily split data across processors.

All sparse matrices are stored in the compressed sparse row (CSR)
format. The CSR format is analagous to the compresses sparse column
format~\cite{1973sparse} with entries stored by row rather than
column. The CSR format consists of three arrays with values stored
sequentially. The total number of elements within these arrays for a
matrix with $n$ rows and $m$ nonzeros is $2m+n+1$.

The total amount of memory required to store all the values used by
the SpMV kernel is called the problem size. The values required are
the three arrays from the CSR representation of the matrix, the array
to store the vector the matrix is being multiplied by (called
$\vec{x}$) and the array storing the result of the multiplication. 

\begin{figure}[htb]
  \centering
  \begin{tabular}{|r|r||r|r|r|} \hline
    Level        & Size  & FD9       & RMAT      \\ \hline
    L2           & 256KB &    18,432 &    18,078 \\
    L3           & 20MB  & 1,474,560 & 1,446,311 \\ \hline
    $16\times$L2 & 4MB   &   294,912 &   289,262 \\
    $2\times$L3  & 40MB  & 2,949,120 & 2,892,623 \\ \hline
  \end{tabular}
  \caption{Maximum number of nonzeros for matrices that fit in each
    cache level for singular caches and all availible caches.}
  \label{fig:cacheSizes}
\end{figure}

The matrices tested have sizes ranging from $8*2^{11} = 16384$
nonzeros to $9*2^{26} = 603,979,776$ nonzeros. The problems range from
being small enough to fit within L2 cache to barely fitting inside
DRAM. Figure~\ref{fig:cacheSizes} shows the maximum NNZ a matrix of
each type may have and still fit within each cache level.

For both FD and R-MAT matrices, the CSR matrix data is very easy for
the system architecture to load. The elements of all three arrays are
stored and accessed sequantially, allowing each memory request to
retreive an entire cache line of useful data. Additionally, if active,
the prefetcher will be able to predict what data will be needed and
retreive it. For FD matrices, $\vec{x}$ exhibits similar behavior. The
three diagonals of three elements each causes the SpMV kernel to
require sequantial access to the elements of $\vec{x}$. Additionally,
the kernel uses each of the elements twice nearly immediately
following the first use. These two properties allow the SpMV kernel to
make effective use of cache, and allow the prefetcher to successfully
anticipate the needs of the kernel. The R-MAT matrices, however, cause
the SpMV kernel to require random elements of $\vec{x}$. The random
pattern causes the prefetcher to fail to get required data, and causes
cache lines to contain mostly useless information. These two
impediments result in the SpMV kernel making many more requests to
DRAM and greatly slowing the computation.






%% In particular, we have been analyzing the SpMV kernel for two types of
%% matrices: one somewhat structured and one highly unstructured.  The
%% somewhat structured matrices are generated using 2D finite difference
%% (FD) method. These matrices consist of three diagonal bands of three
%% elements each, which leads to 9 elements per row. The highly
%% unstructured matrices are synthetically generated R-MAT
%% matrices~\cite{rmat} with an average of 8 elements per row.  R-Mat
%% matrices approximate the sparse matrices produced from network data
%% via a power law distribution and are easy to scale across a range of
%% problem sizes. These matrices have a random structure of nonzeros and
%% little to no data locality in the resulting sparse matrix-dense vector
%% operation. Although these matrices are created randomly, they exhibit
%% a defined skew. This requires non-uniform blocking to achieve optimal
%% performance. For this study, the rows and columns of the R-MAT
%% matrices were randomly permuted. This split the data evenly and
%% allowed a uniform block distribution to achieve the best results. As a
%% baseline for performance comparison, we include data on dense matrices
%% as well. These matrices are constructed to have a similar number of
%% nonzeros (NNZ) to the R-MAT matrices.

%% The matrices range in size, from fitting entirely within L2 
%% cache to barely fitting in DRAM. The smallest matrix has $8*2^{11} = 16384$
%% nonzeros, and the largest has $9*2^{26} = 603,979,776$ nonzeros. Since the matrices used
%% vary slightly in terms of the NNZ they contain, all
%% data is presented on a scale of NNZ.

%% The sparse matrices are stored in Compressed Sparse Row (CSR) format.
%% % TODO reference for CSR format?
%% The dense matrices are stored as flattened arrays. For the
%% matrix-vector multiplication, data from both the matrix and each of
%% the vectors is used and must be kept close to the processor to speed
%% up computation. Figure~\ref{fig:cacheSizes} shows the maximum number
%% of nonzeros a matrix of each type can contain, such that the data for
%% the matrix and vectors used for the SpMV operation are fully contained
%% within the given cache level. % define "problem size"
%% For sparse matrices, this is calculated
%% as the sum of the sizes of the three arrays used for the CSR data
%% storage (one element per row plus two elements per nonzero), the
%% vector being multiplied, and the vector storing the results. For the
%% dense matrices, it is the sum of the size of the flattened matrix, the
%% vector being multplied, and the vector storing the results. All
%% computation is done with double precision floating point numbers. Note
%% that the number of nonzeros is slightly different for the finite
%% difference and R-MAT matrices. This is due to the difference in the
%% number of nonzeros per row\footnote{If an R-MAT matrix (8 elements per
%%   row) and FD matrix (9 elements per row) have the same NNZ, they will
%%   have a different number of rows, so the vectors
  %% that also need to be
  %% stored will be of different sizes.}.


%% \begin{figure}[htb]
%%   \centering
%%   \begin{tabular}{|c|r||r|r|r|} \hline
%%     Level & Size  & Dense     & FD9       & RMAT      \\ \hline
%%     L1    & 32KB  &    64,108 &    36,864 &    36,157 \\
%%     L2    & 256KB &   512,870 &   294,912 &   289,262 \\
%%     L3    & 20MB  & 5,128,706 & 2,949,120 & 2,892,623 \\ \hline
%%   \end{tabular}
%%   \caption{Maximum number of non-zeros for matrices that fit in each cache level for
%%     sixteen threads.}
%%   \label{fig:cacheSizes16}
%% \end{figure}



==> kernels.tex <==
\subsection{SpMV}

%% CUT OUT
%% Useful text from here was incorporated into the introductions section

%% We examine a kernel that is of particular importance to sparse
%% computation and to graph analytics related to network data: sparse
%% matrix-dense vector product.
The sparse matrix-dense vector (SpMV) product is the workhorse kernel
of sparse iterative methods for solving linear systems and eigenvalue
problems (e.g., CG, GMRES, and Krylov-Schur based eigensolvers) and is
often the key computational kernel in these methods, dominating
the runtime. SpMV has been an essential kernel in the signal
processing for graphs work undertaken at MIT Lincoln Laboratory, where
the computation of principal components (obtained through the use of
eigensolvers) is a key step in finding anomalies in network
data~\cite{spg}. 
%% The sparse matrix-matrix product (SpGEMM) is another
%% key kernel for sparse computations, especially computations related to
%% graph analytics. SpGEMM is used in the formation of correlation
%% matrices from adjacency matrices~\cite{byunHPEC2012}, DNA sequence
%% matching, graph clustering, all-pairs shortest-paths
%% algorithms~\cite{alberto}, and algebraic multigrid. SpGEMM is a very
%% challenging kernel and much work has been done in trying to improve
%% its parallel performance~\cite{bulucGEMMexp}. 
For our experiments with
this sparse kernel, we used synthetically generated R-MAT
matrices~\cite{rmat} that approximate the typical graphs present in many applications
involving network data. R-MAT matrices approximate a power law
degree distribution and are straightforward to scale
across a range of problem sizes. 



